Resolved Stellar Mass Maps of Galaxies in the Hubble Frontier Fields: Evidence for Mass Dependency in Environmental Quenching

One of the challenges in understanding the quenching processes for galaxies is connecting progenitor star-forming populations to their descendant quiescent populations over cosmic time. Here we attempt a novel approach to this challenge by assuming that the underlying stellar mass distribution of galaxies is not significantly altered during environmental quenching processes that solely affect the gas content of cluster galaxies, such as strangulation and ram-pressure stripping. Using the deep, high-resolution photometry of the Hubble Frontier Fields, we create resolved stellar mass maps for both cluster and field galaxies, from which we determine 2D S\'ersic profiles, and obtain S\'ersic indices and half-mass radii. We classify the quiescent cluster galaxies into disk-like and bulge-like populations based on their S\'ersic indices, and find that bulge-like quiescent galaxies dominate the quiescent population at higher masses ($M_\star > 10^{9.5}M_\odot$), whereas disk-like quiescent galaxies dominate at lower masses ($10^{8.5}M_\odot< M_\star < 10^{9.5}M_\odot$). Using both the S\'ersic indices and half-mass radii, we identify a population of quiescent galaxies in clusters that are "morphological analogues" of field star-forming galaxies. These analogues are interpreted to be star-forming galaxies that had been environmentally quenched. We use these morphological analogues to compute the environmental-quenching efficiency, and we find that the efficiency decreases with increasing stellar mass. This demonstrates that environmental quenching is more effective on less massive galaxies and that the effect of environment on quenching galaxies is not completely separable from the effect of mass on quenching galaxies.

==> Table2a.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\begin{adjustwidth}{-4.5cm}{}
\footnotesize
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|c|c|c|c|}
\hline
\multicolumn{2}{|l|}{Log Stellar Mass ($M_\star$)}         & \multicolumn{2}{c|}{8.0-8.5}                        & \multicolumn{2}{c|}{8.5-9.0}                        & \multicolumn{2}{c|}{9.0-9.5}                        & \multicolumn{2}{c|}{9.5-10.0}                       & \multicolumn{2}{c|}{10.0-10.5}                      & \multicolumn{2}{c|}{10.5-11.0}                      & \multicolumn{2}{c|}{11.0-11.5}                        & \multicolumn{2}{c|}{11.5-12.0}                        \\ \cline{3-18} 
\multicolumn{2}{|r|}{}                                     & \multicolumn{1}{c|}{min} & \multicolumn{1}{c|}{max} & \multicolumn{1}{c|}{min} & \multicolumn{1}{c|}{max} & \multicolumn{1}{c|}{min} & \multicolumn{1}{c|}{max} & \multicolumn{1}{c|}{min} & \multicolumn{1}{c|}{max} & \multicolumn{1}{c|}{min} & \multicolumn{1}{c|}{max} & \multicolumn{1}{c|}{min} & \multicolumn{1}{c|}{max} & min                       & max                       & min                       & max                       \\ \hline
\multirow{3}{*}{Cluster $n$}              & H band         & 1.64                     & 1.96                     & 1.84                     & 2.03                     & 2.26                     & 2.43                     & 2.80                     & 3.00                     & 3.28                     & 3.52                     & 3.70                     & 4.08                     & \multicolumn{1}{r|}{4.21} & \multicolumn{1}{r|}{5.10} & \multicolumn{1}{r|}{5.21} & \multicolumn{1}{r|}{6.02} \\ \cline{3-18} 
                                          & $\Sigma_\star$ & 1.52                     & 1.77                     & 1.79                     & 1.99                     & 2.37                     & 2.61                     & 2.83                     & 3.09                     & 3.71                     & 3.70                     & 3.34                     & 4.27                     & \multicolumn{1}{r|}{3.43} & \multicolumn{1}{r|}{4.27} & \multicolumn{1}{r|}{3.81} & \multicolumn{1}{r|}{6.42} \\ \cline{3-18} 
                                          & \% diff        & \multicolumn{2}{r|}{-8.478}                         & \multicolumn{2}{r|}{-2.464}                         & \multicolumn{2}{r|}{6.016}                          & \multicolumn{2}{r|}{2.225}                          & \multicolumn{2}{r|}{3.337}                          & \multicolumn{2}{r|}{2.557}                          & \multicolumn{2}{r|}{-17.249}                          & \multicolumn{2}{r|}{-8.838}                           \\ \hline
\multirow{3}{*}{Field $n$}                & H band         & 1.27                     & 1.63                     & 1.18                     & 1.47                     & 1.13                     & 1.35                     & 1.32                     & 1.64                     & 1.47                     & 2.04                     & 2.28                     & 3.95                     & --                        & --                        & --                        & --                        \\ \cline{3-18} 
                                          & $\Sigma_\star$ & 1.35                     & 1.69                     & 1.18                     & 1.31                     & 1.21                     & 1.41                     & 1.40                     & 1.73                     & 1.59                     & 2.34                     & 2.47                     & 4.67                     & --                        & --                        & --                        & --                        \\ \cline{3-18} 
                                          & \% diff        & \multicolumn{2}{r|}{-4.882}                         & \multicolumn{2}{r|}{-5.704}                         & \multicolumn{2}{r|}{5.499}                          & \multicolumn{2}{r|}{5.719}                          & \multicolumn{2}{r|}{11.905}                         & \multicolumn{2}{r|}{14.758}                         & \multicolumn{2}{c|}{--}                               & \multicolumn{2}{c|}{--}                               \\ \hline
\multirow{3}{*}{Cluster $R_{\text{eff}}$} & H band         & 1.43                     & 1.59                     & 1.42                     & 1.59                     & 1.49                     & 1.67                     & 1.89                     & 2.12                     & 2.52                     & 2.8                      & 3.62                     & 4.31                     & \multicolumn{1}{r|}{6.28} & \multicolumn{1}{r|}{8.58} & \multicolumn{1}{r|}{8.27} & \multicolumn{1}{r|}{9.31} \\ \cline{3-18} 
                                          & $\Sigma_\star$ & 1.36                     & 1.52                     & 1.35                     & 1.48                     & 1.41                     & 1.57                     & 1.64                     & 1.80                     & 2.20                     & 2.43                     & 2.97                     & 3.39                     & \multicolumn{1}{r|}{3.81} & \multicolumn{1}{r|}{4.95} & \multicolumn{1}{r|}{4.89} & \multicolumn{1}{r|}{8.62} \\ \cline{3-18} 
                                          & \% diff        & \multicolumn{2}{r|}{-4.403}                         & \multicolumn{2}{r|}{-6.072}                         & \multicolumn{2}{r|}{-5.790}                         & \multicolumn{2}{r|}{-14.171}                        & \multicolumn{2}{r|}{-12.843}                        & \multicolumn{2}{r|}{-19.724}                        & \multicolumn{2}{r|}{-41.080}                          & \multicolumn{2}{r|}{-23.117}                          \\ \hline
\multirow{3}{*}{Field $R_{\text{eff}}$}   & H band         & 2.06                     & 2.37                     & 2.46                     & 2.75                     & 2.72                     & 3.03                     & 2.63                     & 3.01                     & 2.69                     & 3.22                     & 1.71                     & 2.88                     & --                        & --                        & --                        & --                        \\ \cline{3-18} 
                                          & $\Sigma_\star$ & 1.97                     & 2.26                     & 2.35                     & 2.62                     & 2.48                     & 2.76                     & 2.26                     & 2.62                     & 2.13                     & 2.66                     & 1.1                      & 1.89                     & --                        & --                        & --                        & --                        \\ \cline{3-18} 
                                          & \% diff        & \multicolumn{2}{r|}{-4.576}                         & \multicolumn{2}{r|}{-4.775}                         & \multicolumn{2}{r|}{-8.862}                         & \multicolumn{2}{r|}{-13.509}                        & \multicolumn{2}{r|}{-18.839}                        & \multicolumn{2}{r|}{-34.968}                        & \multicolumn{2}{c|}{--}                               & \multicolumn{2}{c|}{--}                               \\ \hline
\end{tabular}
\end{adjustwidth}
\caption{Table displaying values from Figure \ref{fig:IRvsSM2}. The min/max columns are average parameter value per stellar mass bin +/- the standard error, the percent difference between $H-$band light profile and $\Sigma_\star$ distribution profile is also shown. {\color{darkgreen}(Should I format the table like this or format it with average parameter +/- standard error instead?)}\label{table:IRvsSM2}}
\normalsize
\end{table*}

==> Table2b.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\begin{adjustwidth}{-4cm}{}
\footnotesize
\begin{tabular}{|l|r|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
\multicolumn{2}{|l|}{\textbf{Log Stellar Mass ($M_\star$)}}                  & \multicolumn{2}{c|}{\textbf{8.0 - 8.5}} & \multicolumn{2}{c|}{\textbf{8.5 - 9.0}} & \multicolumn{2}{c|}{\textbf{9.0 - 9.5}} & \multicolumn{2}{c|}{\textbf{9.5 - 10.0}} & \multicolumn{2}{c|}{\textbf{10.0 - 10.5}} & \multicolumn{2}{c|}{\textbf{10.5 - 11.0}} & \multicolumn{2}{c|}{\textbf{11.0 - 11.5}} & \multicolumn{2}{c|}{\textbf{11.5 - 12.0}} \\ \hline
\multirow{3}{*}{\textbf{Cluster $n$}}              & \textit{H-band}         & 1.80             & $\pm$0.16              & 1.94              & $\pm$0.09             & 2.35              & $\pm$0.09             & 2.90              & $\pm$0.10              & 3.40               & $\pm$0.12              & 3.89               & $\pm$0.19              & 4.65               & $\pm$0.45              & 5.61               & $\pm$0.41              \\ \cline{3-18} 
                                                   & \textit{$\Sigma_\star$} & 1.65             & $\pm$0.12             & 1.89              & $\pm$0.10             & 2.49              & $\pm$0.12             & 2.96              & $\pm$0.13              & 3.52               & $\pm$0.18              & 3.99               & $\pm$0.28              & 3.85               & $\pm$0.42              & 5.12               & $\pm$1.30              \\ \cline{3-18} 
                                                   & \textit{\% diff}        & \multicolumn{2}{r|}{-8.478}             & \multicolumn{2}{r|}{-2.464}             & \multicolumn{2}{r|}{6.016}              & \multicolumn{2}{r|}{2.225}               & \multicolumn{2}{r|}{3.337}                & \multicolumn{2}{r|}{2.557}                & \multicolumn{2}{r|}{-17.249}              & \multicolumn{2}{r|}{-8.838}               \\ \hline
\multirow{3}{*}{\textbf{Field $n$}}                & \textit{H-band}         & 1.45             & $\pm$0.18              & 1.32              & $\pm$0.14             & 1.24              & $\pm$0.11             & 1.48              & $\pm$0.16              & 1.75               & $\pm$0.28              & 3.11               & $\pm$0.83              & \multicolumn{2}{c|}{--}                   & \multicolumn{2}{c|}{--}                   \\ \cline{3-18} 
                                                   & \textit{$\Sigma_\star$} & 1.52             & $\pm$0.17              & 1.25              & $\pm$0.07             & 1.31              & $\pm$0.10             & 1.57              & $\pm$0.17              & 1.96               & $\pm$0.38              & 3.57               & $\pm$1.11              & \multicolumn{2}{c|}{--}                   & \multicolumn{2}{c|}{--}                   \\ \cline{3-18} 
                                                   & \textit{\% diff}        & \multicolumn{2}{r|}{-4.882}             & \multicolumn{2}{r|}{-5.704}             & \multicolumn{2}{r|}{5.499}              & \multicolumn{2}{r|}{5.719}               & \multicolumn{2}{r|}{11.905}               & \multicolumn{2}{r|}{14.758}               & \multicolumn{2}{c|}{--}                   & \multicolumn{2}{c|}{--}                   \\ \hline
\multirow{3}{*}{\textbf{Cluster $R_{\text{eff}}$}} & \textit{H-band}         & 1.51             & $\pm$0.08              & 1.51              & $\pm$0.08             & 1.58              & $\pm$0.09             & 2.00              & $\pm$0.12              & 2.66               & $\pm$0.14              & 3.96               & $\pm$0.34              & 7.43               & $\pm$1.15              & 8.79               & $\pm$0.52              \\ \cline{3-18} 
                                                   & \textit{$\Sigma_\star$} & 1.44             & $\pm$0.08              & 1.41              & $\pm$0.06             & 1.49              & $\pm$0.08             & 1.72              & $\pm$0.08              & 2.32               & $\pm$0.12              & 3.18               & $\pm$0.21              & 4.38               & $\pm$0.57              & 6.76               & $\pm$1.86              \\ \cline{3-18} 
                                                   & \textit{\% diff}        & \multicolumn{2}{r|}{-4.403}             & \multicolumn{2}{r|}{-6.072}             & \multicolumn{2}{r|}{-5.790}             & \multicolumn{2}{r|}{-14.171}             & \multicolumn{2}{r|}{-12.843}              & \multicolumn{2}{r|}{-19.724}              & \multicolumn{2}{r|}{-41.080}              & \multicolumn{2}{r|}{-23.117}              \\ \hline
\multirow{3}{*}{\textbf{Field $R_{\text{eff}}$}}   & \textit{H-band}         & 2.22             & $\pm$0.15              & 2.61              & $\pm$0.14             & 2.87              & $\pm$0.16             & 2.82              & $\pm$0.19              & 2.96               & $\pm$0.27              & 2.29               & $\pm$0.58              & \multicolumn{2}{c|}{--}                   & \multicolumn{2}{c|}{--}                   \\ \cline{3-18} 
                                                   & \textit{$\Sigma_\star$} & 2.11             & $\pm$0.15              & 2.48              & $\pm$0.13             & 2.62              & $\pm$0.14             & 2.44              & $\pm$0.18              & 2.40               & $\pm$0.26              & 1.49               & $\pm$0.39              & \multicolumn{2}{c|}{--}                   & \multicolumn{2}{c|}{--}                   \\ \cline{3-18} 
                                                   & \textit{\% diff}        & \multicolumn{2}{r|}{-4.576}             & \multicolumn{2}{r|}{-4.775}             & \multicolumn{2}{r|}{-8.862}             & \multicolumn{2}{r|}{-13.509}             & \multicolumn{2}{r|}{-18.839}              & \multicolumn{2}{r|}{-34.968}              & \multicolumn{2}{c|}{--}                   & \multicolumn{2}{c|}{--}                   \\ \hline
\end{tabular}
\end{adjustwidth}
\caption{Table displaying values from Figure \ref{fig:IRvsSM2}. There are bin-averaged parameters along with their standard error, and the percent difference between $H-$band light profile and $\Sigma_\star$ distribution profile is also shown. {\color{darkgreen}(Should I format the table like this or would there be a better way to format it to make it clearer?)}\label{table:IRvsSM2}}
\normalsize
\end{table*}
